$C^0$-inextendibility of the Kasner spacetime

The Kasner spacetime is a cosmological model of an anisotropic expanding universe without matter and is an exact solution of the Einstein vacuum equations Ric(g) = 0. It is manifestly inextendible as a Lorentzian manifold with a twice differentiable metric. In this thesis we proof that it is even inextendible as a Lorentzian manifold with merely continuous metric, which is a stronger statement. We do so by adapting the proof of the $C^0$-inextendibility of the maximal analytically extended Schwarzschild spacetime established by Jan Sbierski.

==> Acknowledgements.tex <==
\section*{Acknowledgements}

I would like to thank my supervisor Jan Sbierski for his continuous commitment and support during the months I spent in Edinburgh writing this thesis. Furthermore, I am grateful to Michael Kunzinger for making my stay in Edinburgh possible by introducing me to Jan's work and supporting my scholarship application.\\
I acknowledge the financial support through the Kurzfristige wissenschaftliche Auslandsstipendium (KWA) of the University of Vienna.
